The Connection between Out-of-Distribution Generalization and Privacy of ML Models

With the goal of generalizing to out-of-distribution (OOD) data, recent domain generalization methods aim to learn "stable" feature representations whose effect on the output remains invariant across domains. Given the theoretical connection between generalization and privacy, we ask whether better OOD generalization leads to better privacy for machine learning models, where privacy is measured through robustness to membership inference (MI) attacks. In general, we find that the relationship does not hold. Through extensive evaluation on a synthetic dataset and image datasets like MNIST, Fashion-MNIST, and Chest X-rays, we show that a lower OOD generalization gap does not imply better robustness to MI attacks. Instead, privacy benefits are based on the extent to which a model captures the stable features. A model that captures stable features is more robust to MI attacks than models that exhibit better OOD generalization but do not learn stable features. Further, for the same provable differential privacy guarantees, a model that learns stable features provides higher utility as compared to others. Our results offer the first extensive empirical study connecting stable features and privacy, and also have a takeaway for the domain generalization community; MI attack can be used as a complementary metric to measure model quality.

==> dp_training.tex <==


\section{Evaluating Differentially-Private Models}
Findings from Section~\ref{sec:evaluation} and \ref{sec:synthetic} establish that stable-feature based learning approaches such as Perfect-Match or Hybrid provide better privacy guarantees as well as utility, thus acting as a defense for mitigating MI attacks without loss in utility. On the other hand, the best known defense for membership inference attacks which is differential privacy is infamous for degrading model utility. Differentially-private (DP) mechanisms require the addition of noise calibrated systematically to hide the contribution of a single data-point during training, thereby providing membership privacy guarantees~\cite{dwork2014algorithmic,abadi2016deep,papernot2016teacher-dp,hamm2016learning-dp}. This addition of noise results in degradation of model utility proportional to the achieved privacy. This raises the question {\em if stable feature-based learning algorithms provide better empirical membership privacy as compared to differentially-private model while preserving model utility.}

To answer this question. we study the change in OOD accuracy and MI attack accuracy of standard training approach such as ERM and stable features-based learning method such as Perfect-Match when trained with differential privacy guarantees as compared to the no-DP setting. We train these models on both the MNIST datasets using the Pytorch Opacus library v0.14. We train the models for varying $\epsilon$ values ranging from 1 to 10 where $\epsilon = 1$ provides the strongest privacy guarantees. Implementation details and the hyperparameters used for the DP training are in Supp. Section~\ref{sup:impl_details}.

\paragraph{Results.} Figure~\ref{fig:dp-mnist} presents the results for Rotated MNIST ~\subref{fig:dp-rmnist} and Fashion-MNIST~\subref{fig:dp-fmnist} for differentially-private ERM and Perfect-Match. $\epsilon=\infty$ indicates the accuracies for the vanilla methods where with no DP guarantees. Our findings are as follows.

\begin{itemize}
    \item The drop in MI attack accuracy for Perfect-Match from $\epsilon=\infty$ to $\epsilon=10$ or even lower is relatively less than that for ERM. This shows that Perfect-Match provides some inherent mitigation or robustness to MI attacks. 
    \item For Rotated Digit MNIST, the empirical membership privacy of Perfect-Match at $\epsilon=\infty$ as measured via the attack accuracy is comparable to that with $\epsilon=5$ and $10$. Although, note that at $\epsilon=\infty$, there is no provable privacy guarantee.
    \item The utility of Perfect-Match is consistently higher than ERM with a significant gap on Fashion-MNIST dataset for larger $\epsilon$ values. This shows that stable-feature based learning algorithms are a promising direction to balance the privacy-utility trade-off for domain generalization tasks.
    
\end{itemize}



\begin{figure}[t]
\centering
\subfigure[Rotated Digit MNIST dataset]{\label{fig:dp-rmnist}
\includegraphics[scale=0.11]{iclr2022/figures/dp_noise/dp_rmnist.pdf}

}
\subfigure[Rotated Fashion MNIST dataset]{\label{fig:dp-fmnist}
\includegraphics[scale=0.11]{iclr2022/figures/dp_noise/dp_fmnist.pdf}

}
\caption{OOD and MI attack accuracy of differentially-private ERM and Perfect-Match algorithms}
\label{fig:dp-mnist}
\end{figure}

==> eval.tex <==
\section{Experimental Setup}
For our empirical study, we select different state-of-the-art training algorithms for domain generalization and popular image datasets used to evaluate the accuracy of these algorithms.

\subsection{OOD Training Methods and ERM}
\label{training_methods}
There are several algorithms proposed for domain generalization~\cite{muandet2013domain,li2018conddomaingen, li2018adversarialfeature, ganin2016dann, li2018adversarialcada, arjovsky2019irm, piratla2020efficient, dou2019masf}. For our experiments, we use recently proposed methods that aim to learn stable features in their training algorithm, have state-of-the-art OOD accuracy on benchmark datasets, and have code available online. For all methods and the respective loss equations, we use $S$ to denote the set of source domains, $N_{d}$ as the total number of samples for domain $d$, $f$ as the classification model, $L_{d}$ as the classification loss, and $x, y$ to represent the data point and its corresponding true class label.

% we allow for common data augmentations like random cropping, horizontal flip, etc.

% by treating the data from such augmentations as i.i.d and merge them with the original train dataset. 

\paragraph{ERM-Baseline:}
    As our baseline, we use the empirical risk minimization approach to train the model, which minimizes the empirical average of loss over training data points. $ \sum_{d \sim S, i \sim N_{d}} L_{d}(f(x_{i}), y_{i}) $

 It treats the data from different domains as i.i.d and simply augments them. This may lead to issues with OOD generalization ~\cite{arjovsky2019irm, peters2016causal} as we need to learn representations that are robust to the changes in the domains. Hence, a variety of approaches (described below) augment the empirical average loss with regularizers to learn domain invariant models. 


\paragraph{Random-Match~\cite{mahajan2020domain,motiian2017ccsa,dou2019masf}.}  Random-Match matches pairs of same-class data points randomly across domains to regularize the model. The idea behind matching across domains is to learn a representations that is invariant to the changes in the source domains, which may lead to better generalization performance. The training loss objective is given by, 

\begin{equation}
\small
\label{eq:erm_match}
\sum_{d \sim S, i \sim N_{d}} L_{d}(h \circ \phi(x_{i}), y_{i}) + \lambda * \sum_{ \Omega(j, k)=1  | j \sim N_{d}, k \sim N_{d'} } Dist(\phi(x_{j}),  \phi(x_{k})) 
\end{equation}

where $\phi$ represents some layer of the network $f=h \circ \phi$, $\Omega$ represents the match function used to randomly pair the data points across the different domains. This may not necessarily enforce learning stable features. 


\paragraph{CSD~\cite{piratla2020efficient}.} Common-Specific Low-Rank Decomposition (CSD) leads to effective OOD generalization by separating the domain specific and domain invariant parameters, and utilizes the domain invariant parameters for reliable prediction on OOD data. It decomposes the model's final classification layer parameters $w$ as $w= w_{s} + W*\gamma$, where $W$ represents the k-rank decomposition matrix, $w_{s}$ represents the domain invariant parameters and $\gamma$ represent the k domain specific parameters. It optimizes empirical average loss with both the domain invariant and domain specific parameters, along with an orthonormality regularizer that aims to make $w_s$ orthogonal to the decomposition matrix $W$. Please refer to Algorithm 1 in their paper~\cite{piratla2020efficient} for more details.
 
\paragraph{IRM~\cite{arjovsky2019irm}.}    
Invariant Risk Minimization (IRM)  aims to learn invariant predictors that simultaneously achieve optimal empirical risk on all the data domains. It minimizes the empirical average loss, and  regularizes the model by the norm of gradient of the loss at each source domain as follows:

\begin{equation}
\small
\begin{split}
 \sum_{d \sim S, i \sim N_{d}} L_{d}(w \circ \phi(x_{i}), y_{i})  + \lambda * \sum_{d \sim S} || \nabla_{w|w=1.0} \sum_{i \sim N_{d}}  L_{d}(w \circ \phi(x_{i}), y_{i})  ||^{2}
\end{split}
\end{equation}


where $f= w \circ \phi$ and $\lambda$ is a hyper parameter. In practice, $\phi$ is taken to be the final layer of the model $f$, (which makes $\phi$ and $f$ to be  the same ). Hence, minimizing the above loss would lead to low norm of the domain specific loss function's gradient and guide the model towards learning an invariant classifier, which is optimal for all the source domains.

    
\paragraph{MatchDG~\cite{mahajan2020domain}.} The algorithm enforces the same representation for pairs of data points from different domains that share the same causal features. It uses contrastive learning to learn a \textit{matching} function to obtain pairs that share stable causal features between them. The loss function for the method is similar to that of Random-Match (Eq~\ref{eq:erm_match}), with $\Omega$ representing the match function learnt by contrastive loss minimization. Hence, the algorithm consists of two phases; where it learns the matching function $\Omega$ in the first phase, and then minimizes the loss function in Eq~\ref{eq:erm_match} during the second phase to learn the final model. Please refer to the Algorithm  1 in Mahajan et al.~\cite{mahajan2020domain} for more details.
    
\paragraph{Perfect-Match~\cite{mahajan2020domain,hendrycks2019augmix}. } Finally, we use an algorithm that can be considered to learn \textit{true stable} features for given data, since it relies on knowledge of true base object for a subset of images (and thus guaranteed shared causal features between them). This approach again has a similar formulation to Eq~\ref{eq:erm_match}, where the match function $\Omega$ is satisfied for data points from different domains that share the same base causal object. Hence, it aims to learn similar representations for two data points that only differ in terms of the domain specific 
attributes.  

\paragraph{Hybrid~\cite{mahajan2020domain}.}
Perfect matches as explained above are often unobserved but given through Oracle access. However, in real datasets, augmentations can also provide perfect matches, leading to the \textit{Hybrid} approach using both the MatchDG and augmented Perfect-Match. It learns two match functions, one on the different source domains as per MatchDG, and the other on the augmented domains using Perfect-Match. 


Note that Perfect-Match is an ideal training algorithm that assumes knowledge of ground-truth matches across domains, and therefore cannot be applied in real-world settings. In contrast, the Hybrid algorithm depends on creating matches of the same base object using self-augmentations and can be used practically whenever augmentations are easy to create (such as in image datasets). In the experiments that follow, we use the PerfectMatch algorithm for the simulated Rotated-MNIST and Fashion-MNIST datasets, where it should be considered as an ideal method. For the real-world Chest X-rays dataset, we use the practical Hybrid algorithm since we have no knowledge about the true perfect matches. 

\subsection{Datasets}
\label{sec:datasets}
\begin{table*}[t]
\centering
\caption{Dataset details}
\label{tab:dataset_details}
\begin{tabular}{l |ccccc@{}}
\toprule
Dataset                                                  & Total Classes                   & Total Domains          & Source Domains                   & Target Domains               & Samples per Domain                \\ \midrule

Rotated-MNIST &     10                  &       7                               &  $15^{\circ}$, $30^{\circ}$, $45^{\circ}$, $60^{\circ}$, $75^{\circ}$               &  $0^{\circ}$, $90^{\circ}$    & 2000                                                                \\ 
                                                                                  
Fashion-MNIST &     10                  &        7                       &   $15^{\circ}$, $30^{\circ}$, $45^{\circ}$, $60^{\circ}$, $75^{\circ}$                     &  $0^{\circ}$, $90^{\circ}$                     &    10000               \\ 

ChestXray   &       7       &            3           &  NIH, ChexPert &      RSNA                 &     Table~\ref{tab:chestxray_details}                                                            \\

\bottomrule
\end{tabular}
\end{table*}

\begin{table}[t]
\centering
\caption{Train/Val/Test splits for the ChestXRay dataset.}
\label{tab:chestxray_details}
\begin{tabular}{l |ccc@{}}
\toprule
Domain  & Training Set                  & Validation Set          & Test Set  \\ \midrule

NIH & 800  &  200  &  430 \\ 
                                                                                  
ChexPert & 2618  &   654   &  1402 \\ 

RSNA  & 3367  & 841  &  1803  \\

\bottomrule
\end{tabular}
\end{table}

%This results in learning feature representations that lead to good generalization on out of domain dataset.
%We evaluate on the following two domain generalization datasets.

\paragraph{Rotated-MNIST.}  
This dataset is built upon the MNIST handwritten digits, where we create multiple domains by rotating each digit with the following angles $0^{\circ}$,  $15^{\circ}$, $30^{\circ}$, $45^{\circ}$, $60^{\circ}$, $75^{\circ}$, $90^{\circ}$ ~\cite{ghifary2015multitaskae}. Angles from $15^{\circ}$ to $75^{\circ}$ constitute the source domains for training and  the angles $0^{\circ}$ and $90^{\circ}$ are the unseen test domains.
Here, the different images across domains share the same base causal object and provide access to true matches required for Perfect-Match approach. Following~\cite{piratla2020efficient}, we sample $2000$ data points for each domain, which contribute to the train/test dataset and use ResNet-18 models for classification. To create validation set, for each domain we sample additional data points and makes its size as 20\% of the training size.

\paragraph{Fashion-MNIST.}

This dataset~\cite{xiao2017fashion} has the same structure as MNIST, where it replaces the handwritten digits by fashion items. We follow the same setup as above for Rotated-MNIST, except we sample $10,000$ data points per domain. 

\paragraph{ChestXRay.}
To evaluate on a more practical scenario, we use the dataset of 
Chest X-rays images from ~\cite{mahajan2020domain}, that comprises of data from different hospital systems: NIH~\cite{wang2017chestx}, ChexPert~\cite{irvin2019chexpert} and RSNA~\cite{rsna}. The task is to train a classifier that predicts whether a patient suffers from Pneumonia or not. To simplify the analysis, we remove the class imbalance from each of the three domains. For each domain, we sample all the images corresponding to class (1), divide them as 30\% for test set and the rest for the train set of that domain. Also, we create a validation set for each domain by further sampling 25\% of the training set. Then for all the various splits on each domain, we randomly sample images corresponding to class (0) to ensure to class imbalance.

We use the domains (NIH, ChexPert) for training and the unseen domain (RSNA) for evaluation (details in Table~\ref{tab:chestxray_details}). Note that this dataset contains spurious correlation in the source domains due to a vertical translation that shifts all the data points in source domains corresponding to class label 0 downwards.  This creates a downward shift in the position of lungs for the images with class (0) as compared to the image with class (1), which creates the spurious feature as the difference in the position of lungs. No such spurious correlation is present in the target domain. Thus, the setup penalizes models that rely on spurious correlations for making predictions, as they would get high accuracy on the source domains, while they would fail on the target domains as no such translation exists in the case of test images.

\subsection{Implementation Details}

We follow the same procedure as in~\cite{mahajan2020domain} for the OOD training and evaluation of methods. %The complete details for the same can be found the supplementary section B of their work~\cite{mahajan2020domain}. 
To summarize, we use the model ResNet-18 (no pre-training) for the Rotated-MNIST and Fashion-MNIST dataset, and we use pre -trained DenseNet-121 for the ChestXRay dataset. For the matching based methods (Random-Match, MatchDG, Perfect-Match), we use the final classification layer of the network as $\phi$ and  for the matching loss regularizer (Eq~\ref{eq:erm_match} ). For all the methods across datasets, we use Cross Entropy for the classification loss ($L_{d}$), and use SGD to optimize the loss. Also, we use the data from the source domains for validation and never expose the model to any data from the target domains while training. The details regarding the train/validation/test splits for each dataset are described in the section~\ref{sec:datasets} and Table~\ref{tab:dataset_details}.

\paragraph{Source code.} Our source code is available at the link in the footnote~\footnote{https://anonymous.4open.science/r/3cd41059-40a6-4fba-a966-d1c05c6f8573/}. All the datasets used in our experiments are publicly available to download. 


\paragraph{Membership Inference (MI) Attacks.}
For implementing MI attacks, we first create the attack-train and attack-test dataset from the original train and test dataset for the ML model. We first sample $N$ number of data points ( N: $2,00$ for Rotated-MNIST, $10,000$ for Fashion-MNIST, N: $1,000$ for ChestXRay  ) from both the original train and test dataset to create the attack-train dataset. Similarly, we sample an additional set of $N$ data points from original train, test dataset to create the attack-test dataset. 


For the Classifier-based attack, we label the data points from the training dataset as members, and the data points from the test dataset as non members. We then train a 2-layer fully-connected network ( with hidden dimensions 8, 4 respectively ) to distinguish members from non-members for all the models and datasets. We use Adam Optimizer with learning rate 0.001, batch size 64 and 5000 steps / 80 epochs.

For the Loss-based and Entropy-based attack, we first identify the threshold $\tau$ as the max loss/entropy score among all the members in the attack-train dataset, and then scale the threshold by an integer value $s$ chosen randomly from the grid $(1, \tau)$. We then evaluate the performance for the different threshold obtained by scaling, and choose the final threshold as the one that gives the highest classification accuracy on the attack-train dataset. We use the final theshold to evaluate performance on the attack-test dataset. We sample 10 values at random for the scaling factor $s$ for our experiments across datasets. Also, if the initial threshold $\tau$ is less than 10 (which would restrict from sampling 10 distinct integers from the grid defined above), we update the grid to be $(1, 20)$ from $(1, \tau)$.


\paragraph{Attribute Inference (AI)  Attacks.}
We use all the source and target domains, and sample data points from their training/test set to create the attack-train/attack-test dataset respectively. We then label data points in the attack-train and attack-test dataset based on the attribute, and then train a classifier to discriminate among different attributes. We follow the same procedure for training the classifier as defined for the Classifier-based attack above.

==> methodology.tex <==

\section{Preliminaries and Metrics}
We evaluate the privacy and generalization properties of a training method using four different metrics: membership inference accuracy, attribute inference accuracy, out-of-domain task accuracy, and stability of features as measured by the mean rank metric for  learned representations. % that allows us to measure stability of features.

\subsection{Membership Inference (MI) Attacks }
Several methods have been proposed in the literature to compute MI attack accuracy based on the threat-model i.e., black-box or white-box and computational power of the attacker. All these methods identify the boundary that helps to distinguish between members and non-members. As our goal is to use MI attack accuracy as a measure for privacy, we select three different methods that are popularly used in the literature. 

For all the different attack techniques, we first create an attack train and attack test dataset using a subset of the original training and test dataset used by the ML model. Thus, our attack accuracy results are an upper bound for all the training techniques. We then infer the parameters (output probabilities) required for the privacy attack to classify members from non members on the attack train dataset, and evaluate its  performance on attack test dataset. 


\paragraph{Classifier-based attack~\cite{shokri2017membership}} The classifier based attack was first proposed in the seminal work by Shokri et al.~\cite{shokri2017membership} and has been used commonly in several works to demonstrate membership inference attacks~\cite{updates-leak,salem2018ml,zhang2020dataset,song2020Overlearning}. In this method, the adversary trains a classifier, often called as a meta-classifier or an attack classifier to predict member vs. non-member. The input for this classifier is generated by training several shadow models that are trained in a similar fashion as the target model. The output probability vector of several known members and non-members from these shadow models is provided as input for training the classifier. 

Instead of training shadow models, we assume access to a subset of training dataset and directly query the target model to generate the input features for the attack classifier. The upper bound works for us since our goal is to perform a relative comparison of different training technqiues using the MI attack. 


\paragraph{Loss-based attack~\cite{yeom2018privacy}}
Instead of training shadown models, Yeom et al. proposed MI attack that relies on the loss of the target model. The attacker observes the loss values of a few samples and identifies a threshold that distinguishes members from non-members. The intuition is that training data points will have a lower loss value as compared to test data points.
This attack is computationally cheap and the attacker does not need to train shadow models or an attack classifier. However, the attack assumes access to the loss values of the target model i.e., it requires white-box access to the model. 


\paragraph{Prediction Entropy-based attack~\cite{salem2018ml,song2020systematic}.}
The last method we use was first proposed in Salem et al.~\cite{salem2018ml} and recently improved by Song et al.~\cite{song2020systematic}. This method uses the prediction entropy computed from the probability vector to identify a threshold that distinguishes between members and non-members. For each data point, we predict members vs non members by checking whether the entropy score is below a certain threshold or not. This method improves on both the above method as it is computationally cheap i.e., does not require training a classifier and works in a black-box setting.


\subsection{Attribute (Property) Inference (AI) Attacks }
Recently, several attacks have demonstrated the machine learning models can leak attribute values or properties of input data that are simply correlated but not relevant for the desired prediction task~\cite{Melis2019Exploiting,ganju2018property,song2020Overlearning,zhang2020dataset}. Song et al. show that this because of overlearning the model which then utilizes correlated features for the prediction task instead of stable features. Such correlated features may be sensitive but not directly a predictor of the final task. Zhang et al. ~\cite{zhang2020dataset} show that such correlated attributes can be leaked even if they are removed or ignored during the training because of their correlation to other features. 

We use a classifier-based attribute inference attack as our second metric to evaluate the privacy of different  training techniques that aim for domain generalization. The attack is similar to the MI classifier attack, where we query a subset data points to the target model and use their prediction probability vector as input feature for the attack classifier. The ground truth is the value of the sensitive attribute for the given input. The classifier is trained to predict the attribute value for a given input feature of probability vector. This attack works in a black-box setting.

With the goal to evaluate domain generalization training techniques, we consider two scenarios in our attribute inference attack. In the first case, we consider the domain itself a as a sensitive attribute and for the second case, we introduce a synthetic attribute that is equally present in all the domains and has a correlation with the output class.

\subsection{Out-of-Domain Accuracy}
To understand the generalization ability of a training technique, we use the accuracy as a measure when computed on inputs that are generated from domains that are {\em not} seen during training. This is different than standard test accuracy measure where often the validation and test data have the same distribution.  Since our goal is to understand the connection between domain generalization techniques and privacy, we select out-of-domain accuracy as one of our evaluation metrics.

\subsection{Measuring Stable Features}
%\shruti{Explain why is mean rank a good metric to measure stable features. Add mean rank equation}
Measuring stability of learnt features is a hard task, since the ground-truth stable features are unknown for a given classification task. For example, in a MNIST task to classify the digit corresponding to an input image, the shape of the digit can be considered as the stable (or causal) feature whereeas its color or rotation are not stable features. Even if stable features are known, in image datasets, they are typically high-level features (such as shape) that themselves need to be learnt from data. Therefore, verifying stable features directly is a non-trivial task. 

Instead, we use the property described by causal domain generalization work~\cite{mahajan2020domain,heinze2017conditional} that input images that share the base object have the same stable (or causal) features. Thus, if we can select pairs of inputs with the same base object, then they should share the same causal features. Such a pair is known as a \textbf{perfect match}. Note that a base object refers to the same semantic input such as a person or a handwritten digit. Input images may consist of the same person in different views or the same handwritten digit in different colors or rotations, but their base object remains the same. Note that there is a many-to-one relationship between an object and its class label. Each class label consists of many objects, which in turn consist of many input images that are differentiated by certain non-stable features like view or rotation or noise.  

We use the above property to construct a ranking metric for any ML model. We consider the last layer (logit) representation of the ML model and use a standard distance metric to represent similarity between any two inputs by comparing their representation distances. Then, for each image in the dataset for which a ground-truth perfect match is known, we compute the rank of its ground-truth perfect match based on the ML model's representation.  Lower rank is better: a rank of 1 indicates that the learnt feature representation accurately captures the perfect matches, and thus is consistent with a representation based only on stable features (at least on the known perfect matches). 

%For datasets that contain perfect matches/augmentations, we can compute the  feature stability using metrics mentioned in  ~\cite{mahajan2020domain}. We evaluate on one of such match function metrics, the mean rank metric. To compute mean rank metric, for each data point we maintain a sorted list by computing its distance among all the data points in another domain, and check for the rank of its perfect match in the other domain among the sorted list. 


Formally, the mean rank metrics is computed as follows. For the matches (j, k) as per the ground-truth perfect match strategy $\Omega$, compute the mean rank for the data point j w.r.t the learnt match strategy $\Omega^{'}$ i.e. $S_{\Omega^{'}}(j)$

\begin{equation}
     \frac{\sum_{\Omega(j,k)=1; d\neq d'}  Rank[ k \in S_{\Omega^{'}}(j) ] }{\sum_{\Omega(j,k)=1; d\neq d'} 1}
\end{equation}    

The efficacy of the mean rank metric depends on the ground-truth perfect matches. For simulated datasets like Rotated-MNIST and Fashion-MNIST, we know the ground-truth matches for each input and use that to evaluate the mean rank metric (the same matches are not provided to the DG methods, except to the ideal Perfect-Match method). For the real-world Chest X-rays dataset, we instead construct self-augmentations for each image by utilizing common transformations like flip from the computer vision literature. We use these self-augmentations as perfect matches (again, these matches are not provided to the DG methods except for the Hybrid method, which has access to them).
